Pricing Cryptocurrency Options

Cryptocurrencies, especially Bitcoin (BTC), which comprise a new digital asset class, have drawn extraordinary worldwide attention. The characteristics of the cryptocurrency/BTC include a high level of speculation, extreme volatility and price discontinuity. We propose a pricing mechanism based on a stochastic volatility with a correlated jump (SVCJ) model and compare it to a flexible co-jump model by Bandi and Ren\`o (2016). The estimation results of both models confirm the impact of jumps and co-jumps on options obtained via simulation and an analysis of the implied volatility curve. We show that a sizeable proportion of price jumps are significantly and contemporaneously anti-correlated with jumps in volatility. Our study comprises pioneering research on pricing BTC options. We show how the proposed pricing mechanism underlines the importance of jumps in cryptocurrency markets.

==> econometrics_aj_1029.tex <==
\section{The BTC dynamic}

% The CRyptocurrency IndeX \includegraphics[scale=0.037]{figures/crix1} developed by \cite{hardle2015crix} provides a market measure which consists of a selection of representative cryptos. Through the exceptional channel of an ICO, a CC startup can bypass the rigorous and regulated capital-raising process required by venture capitalists or banks. The appendix lists the top 10 constituents used to construct the CRIX index. The mechanism of selecting CRIX constituents is explained in \cite{trimborn2018}.

The dynamics of BTC prices depicted in Figure \ref{fig:BTCprice} give us a glimpse of its evolution.  A dramatic surge was observed after March 2017 due to widespread interest in cryptocurrencies (CCs). The subsequent drop in June was caused by a sequence of political interventions. Indeed, several governmental announcements of bans on initial coin offerings (ICOs), for example, have spurred intensive movements on CC markets.\\

\begin{figure}[htp]
\caption {BTC Prices and Returns}\label{fig:BTCprice}
\begin{center}
\begin{tabular}{cc}
%\includegraphics[scale=0.4]{figures/crix_price.pdf} &
%\includegraphics[scale=0.4]{figures/crix_return.pdf}  \\
\includegraphics[scale=0.4]{figures/btc_price.pdf} &
\includegraphics[scale=0.4]{figures/btc_return.pdf}  \\
\end{tabular}
\end{center}
\footnotesize
\textit{Notes}: This figure graphs the BTC daily price (left panel) from 31/07/2014 to 29/09/2017 and BTC returns (right panel). The returns ($R_t$) are calculated as
%\begin{equation*}
    $R_t=ln(P_t)-ln(P_{t-1})$, where $P_t$ is the BTC price at time $t$.
%\end{equation*}
\end{figure}

Figure \ref{fig:BTCprice} indicates that BTC prices do not behave like conventional stock prices. One records extremely high volatility and scattered spikes. These prices are far from being stationary. % The plot of returns shows that volatility is time-varying and clustering. Therefore we start to fit the returns of BTC with the GRACH model. 
%The differentiation and detrending, or change point detection are required.  After an inspection through the ACF and PACF plot in Figure \ref{fig:acf}, we start with an ARIMA($p, d, q$) model,
%\begin{equation}
       a(L)\Delta y_{t}= b_{L}\varepsilon_{t}
\end{equation}
%where $y_{t}$ is the variable of interest, $\Delta y_{t}= y_{t}- y_{t-1}$, $L$ is the lag operator and $\varepsilon_{t}$ a stationary error term. Model selection criteria such as AIC or BIC indicates that the ARIMA($2, 0, 2$) is the model of choice. The parameters estimated from the ARIMA(2,0,2) are reported in Table \ref{tab:arima}. The significant negative signs in $a_1$ and $a_2$ indicate an overreaction, that is, a promising positive return today leads to a return reversal in the following two days or vice versa. Hence, the CC markets tend to overreact to good or bad news, and this overreaction can be corrected in the following two days. An ARIMA model for the CC assets, therefore, suggests predictability due to an ``overreaction''.
